Understanding Domain-Size Generalization in Markov Logic Networks

We study the generalization behavior of Markov Logic Networks (MLNs) across relational structures of different sizes. Multiple works have noticed that MLNs learned on a given domain generalize poorly across domains of different sizes. This behavior emerges from a lack of internal consistency within an MLN when used across different domain sizes. In this paper, we quantify this inconsistency and bound it in terms of the variance of the MLN parameters. The parameter variance also bounds the KL divergence between an MLN's marginal distributions taken from different domain sizes. We use these bounds to show that maximizing the data log-likelihood while simultaneously minimizing the parameter variance corresponds to two natural notions of generalization across domain sizes. Our theoretical results apply to Exponential Random Graphs and other Markov network based relational models. Finally, we observe that solutions known to decrease the variance of the MLN parameters, like regularization and Domain-Size Aware MLNs, increase the internal consistency of the MLNs. We empirically verify our results on four different datasets, with different methods to control parameter variance, showing that controlling parameter variance leads to better generalization.

==> _old_06_rbm.tex <==
\section{Relational block model}

% \red{
%   \begin{itemize}
%     \item Text: Motivate RBM
%     \item Motivate maximum Likelihood learning
%   \end{itemize}
% }
In this section we introduce the Relational Block Model (RBM). We will then show that any projective MLN in the two variable fragment is an RBM.
\begin{definition}
  \label{def: RBM}
  Let $n$ be a positive integer (the number of domain constants), $u$ be a
  positive integer (the number of 1-types), $b$ be a positive integer (the number of 2-tables), $p = (p_1,...,p_u)$ be a probability vector on $[u]=\{1,...,u\}$ 
  and $W  = (w_{ijl}) \in [0,1]^{u\times u \times b}$, where $w_{ijl} = w_{\underline{ijl}}$  ($w_{ijl}$ is the conditional probability of domain elements $(c,d)$ realizing the $l^{th}$ 2-table, given $ {i(c)}$ and $ {j(d)}$).
  The multi-relational graph $(X,Y)$ is drawn under $\mathrm{RBM}(n,p,W)$ if $X$ is an $n$-dimensional vector with $i.i.d$ components distributed under $p$ and $Y$ is a random vector with its component $y_{qr} = l$, where $l \in [b]$, with a 
  probability $w_{x_qx_rl}$ independently of all other pair of domain constants. 
  
  % \red{We also define $k_i = k_i(X) = |\{x_q: x_q = i \}| $ and 
  % $h^{ij}_l = h^{ij}_l(Y) = |\{y_{qr}:x_q = i, x_r = j \text{ and }y_{qr} = l\}|$.}
  
  Thus, the probability distribution of $(X,Y)$ is defined as follows, where $\x \in [u]^{n}$ and $\y \in [b]^{\binom{n}{2}}$ 
\begin{align*}
  P(X=\x) &:= \prod_{q=1}^{n} p_{x_q} = \prod_{i=1}^{u} p_{x_i}^{k_i}\\
  P(Y=\y|X = \x) &:= \prod_{1\leq q < r \leq n  } w_{x_qx_ry_{pq}} \\
  &= \prod_{ 1\leq i \leq j \leq u} \, \prod_{1\leq l \leq b}(w_{ijl})^{h^{ij}_l}
\end{align*}
 
\end{definition}

% Notice that an RBM is essentially a Labelled Stochastic Block Model \cite{SBM_ebbe}.  Furthermore, it can be seen that an RBM can be expressed as an MLN of the form 
% \begin{equation}
%   \label{eq: RBM_2_MLN}
% \{(i(x),\log p_i)\} \cup \{(ijl(x,y),\log w_{ijl})\} 
% \end{equation}
% \begin{remark}
% Notice that RBMs allow $p_i$ and $w_{ijl}$ to be $0$, making the conversion to MLN slightly problematic. But this problem can be mitigated by simply excluding the 1-types from the set of 1-types for which $p_i = 0$ and by defining the set of 2-tables conditionally on 1-types. A similar approach can be used to restrict $\Omega^{(n)}$ to the set of models of an FO$^2$ formula. We do not take this approach as it makes the notation cumbersome without changing the essence of the results. 
% \end{remark}

% In previous works \cite{Projectivity_first} on projectivity, it was shown that simple notions  like homophily in a graph may not be modelled as a projective MLN. 

In the following example, we show how RBMs can model homophily. 

\begin{example}[Homophily] Let us have an FO$^2$ language with a unary predicate $C$ (representing a two colors) and a binary predicate $R$. 
  We wish to model a distribution on simple undirected graphs i.e. models of the formula $\phi = \forall xy. \neg R(x,x) \land (R(x,y) \rightarrow R(y,x))$ such that 
  same color nodes are more likely to have an edge. Due to $\phi$ the 1-types with $\neg R(x,x)$ as a conjunct have a probability zero. Hence, we can assume we have only two 1-types:
  $1(x) = C(x)\land \neg R(x,x) $ and $2(x) = \neg C(x)\land \neg R(x,x) $ (representing two possible colors for a given node). Similarly due to $\phi$, we have only two 2-tables $1(x,y): R(x,y) \land R(y,x)$ and $ 2(x,y): \neg R(x,y) \land \neg R(y,x)$ (representing existence and non existence of edges). We can now easily define homophily by following parameterization of an RBM.
  $p_1 = p_2 = 0.5$ i.e. any node can have  two colors with equal probability. Then we can define $w_{111} = 0.9$, $w_{112} = 0.1$, $w_{221} = 0.9$, $w_{222} = 0.1$, $w_{121} = 0.1$ and $w_{122}=0.9$. 
\end{example}

% We will now show that any projective MLN in the two variable fragment is equivalent to an RBM.
\begin{theorem}
  \label{th:RBM_MLN}
  Every projective Markov Logic Network in the two variable fragment is an RBM.
\end{theorem}
\begin{proof}
  The proof follows from the sufficiency proof in Lemma \ref{lem: sufficiency_factorisation}. Notice that in the proof, we derive equation \eqref{eq: RBM}, which is exactly the expression for RBM.
\end{proof}









==> _old_07_learning.tex <==
\section{Maximum Likelihood Learning}
In a learning setting, for an MLN $\{\phi_i,a_i\}$ in the two variable fragment, we are interested in estimating the set of parameters $\bm{\theta} = \{a_i\}$
that maximize the likelihood of a training example such that the learnt MLN is projective. As analyzed in \cite{one_Network,Relational_Marginal_Polytope}, we will focus 
on the scenario where only a single possible world $\omega \in \Omega^{(n)}$ is observed. We estimate $\bm{\theta}$ by maximizing the likelihood
\begin{equation}
    \label{likelihood}
    L^{(n)}(\bm{\theta}|\omega) = P^{(n)}_{\bm{\theta}}(\omega)
\end{equation}


Notice that although every projective MLN can be equivalently defined as an RBM. The Maximum Likelihood  parameter estimate for an RBM is not the same as the  parameter estimate for an MLN such that it is projective. 

We will now provide, the maximum likelihood estimator for an RBM. This estimator is completely analytically definable and admits many desirable consistency and efficiency properties. We will then show that, as far as maximizing data likelihood is concerned, RBM is at least as good as any projective MLN.


\begin{proposition}
    \label{lem: RBM_ML}
    Given a training example $\omega \in \Omega^{(n)}$, the maximum likelihood parameter estimate for an RBM is given as :
    \begin{align}
        p_i = \frac{k_i}{n}    
        & &w_{ijl} = \frac{h^{ij}_l}{\bk(i,j)}
    \end{align}
\end{proposition}
Proposition \ref{lem: RBM_ML} can be derived by maximizing the log likelihood due to the distribution given in Definition \ref{def: RBM}. 



We will now see how maximum likelihood parameter estimate can be obtained for an MLN such that the MLN is projective. 

Given an MLN $\{\phi_i,a_i\}_i$ in the two variable fragment, where $\bm{\theta} = \{a_i\}_i$ are unknown parameters to be estimated, due to Theorem \ref{MLN_Normal_Form}, we can define $s_i(\bm{\theta})$ and $t_{ijl}(\bm{\theta})$, such that the likelihood is given as:

\begin{equation}
L(\omega|\bm{\theta}) = \frac{1}{Z(n)} \prod_{i \in [u]} s_{i}(\bm{\theta})^{k_i} \prod_{\substack{i,j\in [u]\\ i \leq j}}\prod_{l \in [b]} (t_{ijl}(\bm{\theta}))^{h^{ij}_l}
\end{equation}
The maximum likelihood parameter estimates such that the estimated MLN is projective,  can be then obtained by solving the following optimization problem:
\begin{align}
    \label{MLN_ML_proj}
    \begin{split}
       \text{ maximize:}  &\Big[ \sum_{i\in [u]}k_i \log s_{i}(\bm{\theta}) + \sum_{\substack{i,j \in [u] \\ i \leq j }}\sum_{l\in [b]}h^{ij}_l\log{t_{ijl}(\bm{\theta})} \\
        & - n\log\big( \sum_{i\in [u]} s_{i}(\bm{\theta}) \big) - \binom{n}{2} \log f_{11} \Big]\\
        \text{ subject to:  } &\forall i,j,i',j' \in [u] : f_{ij} = f_{i'j'}         
    \end{split}
       %& +  \lambda (1 - \sum_{i\in [u]}p_i) - \sum_{\substack{i,j \in [u] \\ i\leq j}} \lambda_{ij} (1 - \sum_{l\in [b]}w_{ijl}) 
\end{align}
Notice, that $- n\log\big( \sum_{i\in [u]} s_{i}(\bm{\theta}) \big) - \binom{n}{2} \log f_{11}$ represents $-\log(Z(n))$ and $f_{11}$ could have been any particular $f_{ij}$ (see \eqref{eq: partition_factorises}). The above optimization can be solved through any conventional optimization algorithm. It can be seen that this problem has a much lesser overhead as far as computing $\log(Z(n))$ is concerned. But the additional constraints may counter act this gain.

% \td{Is it clear that $\bk(i,j)$ is defined w.r.t $\omega$}\\
% \td{proof in appendix}\\



\begin{proposition}
    \label{prop: RBM_best}
    Given a training example $\omega \in \Omega^{(n)}$, then there is no parameterization for any projective MLN in the two variable fragment that has a higher likelihood for 
    $\omega$ than the maximum likelihood RBM for $\omega$.
\end{proposition}
\begin{proof}
    Let $L$ be the likelihood of $\omega$ due to the maximum likelihood RBM. Let $L'$ be the likelihood of $\omega$ due to a projective MLN $\Phi$, such that $L' > L$. Now, due to Theorem \ref{th:RBM_MLN}, $\Phi$ can be expressed as an RBM. Hence, we can have an RBM such that the likelihood of $\omega$ is $L'$, but $L' > L$ which is a contradiction. Hence, we cannot have a projective MLN that gives a higher likelihood to $\omega$ than the maximum likelihood RBM.
\end{proof}
Proposition \ref{prop: RBM_best} shows us that if a data source is known to be projective (i.e. we know that marginals in the data will be independent of the domain at large) then in terms of likelihood, specially in the case of large relational datasets, we are better off in using an RBM than an expert defined MLN. This can also be argued 
from efficiency point of view as RBMs admit much more efficient parameter estimates.


We will now move on to the question: \emph{are  parameters learned on a domain of size $n$, also good for modelling  domain of a different size $m$ ?} This question is an abstraction of 
many real world problems, for example, learning over relational data in presence of incomplete information \cite{social_Network_missing}, modelling a social network from only  sub-sampled populations \cite{social_Network_sample}, modelling progression of a
disease in a population by only testing a small set of individuals \cite{test_disease} etc. 

Jaeger and Schulte \cite{Projectivity_first} formalized the afore mentioned notions in the following two criterions:

\begin{align}
    \label{eq:consistency_1}
    E_{\omega}[\argmax_{\bm{\theta}} \log L^{(m)}(\bm{\theta}|\omega')] &= \argmax_{\bm{\theta}} \log L^{(n)}(\bm{\theta}|\omega) 
\end{align}
\begin{align}
\label{eq: consistency_2}
    \argmax_{\bm{\theta}} E_{\omega}[\log L^{(m)}(\bm{\theta}|\omega')] &= \argmax_{\bm{\theta}} \log L^{(n)}(\bm{\theta}|\omega)
\end{align}

It is easy to see, by law of large numbers, that RBMs satisfy both these criterions. On the other hand the same can not be said about the maximum likelihood estimates for projective MLNs as described in  \eqref{MLN_ML_proj}. 
% Let $\bm{\theta}^{*} \in \Theta$ be the parameter estimate obtained by maximizing \eqref{likelihood} over a world $\omega \in \Omega^{(m)}$. Let $\omega' \in \Omega^{(n)}$ be a larger $n$-world such that $\omega' \downarrow I = \omega$  for sum $I \subset [n]$, where $|I |= m$. Let $\bm{\theta}^{**} \in \Theta$ be the parameter estimate obtained by maximizing $P^{(n)}_{\theta}(\omega')$ for a world $\omega' \in \Omega^{(n)}$ .We would be interested in understanding (i) The relationship between maximum-likelihood parameter estimates $\bm{\theta}^{*}$ and $\bm{\theta}^{**}$ (ii) the complexity of estimating 
% $\theta^{**}$ for P-MLN and RBM.

% Given that an $m$-world $\omega$ is observed as the sub-sample of a larger $n$-world $\omega'$, where the data in $\omega'$ that is not contained in $\omega$ is missing at random \cite{MAR}. Then the marginal likelihood $ML(\bm{\theta}|\omega)$ is simply defined as $P^{(n)}_{\bm{\theta}} \downarrow [m](\omega')$


% In this section we derive the maxim
% \begin{equation*}
% \sum_{i\in[u]}k_i  \log{p_i}  + \sum_{i\leq j \in [u]} \sum_{l\in[b]} h^{ij}_l \log{w_{ijl}} 
% \end{equation*}
% \begin{theorem}
%     10 HOLDS
% \end{theorem}
% \begin{proof}
%    % \sum_{i\in [u]}k_i
% \end{proof}



% \td{THINK ABOUT COMPLEXITY OF LEARNING P-MLN}\\
% \td{Minimum change required to make MLN projective, KL-Divergence?}

% \begin{example}
%     Let us have an MLN $\{C(x) \lor E(x,y): \log w\}$ our goal is to learn $w$ from an $\omega \in \Omega^{(n)}$ such that the MLN is projective. Let us define the following order on 1-types as: $1(x):= C(x)\land E(x,x)$, $2(x):= \neg C(x)\land  E(x,x)$, $3(x):=  C(x)\land \neg E(x,x)$ and $4(x):= \neg C(x)\land \neg E(x,x)$. We define the 2-tables as:  $1(x,y) := E(x,y) \land E(y,x)$, $2(x,y) := E(x,y) \land \neg E(y,x)$, $3(x,y) := \neg E(x,y) \land E(y,x)$ and $4(x,y) := \neg E(x,y) \land \neg E(y,x)$. Hence, $s_1 = w$, $s_2=w$, $s_3 =w$ and $s_4 = 1$. Also, w_{}
% \end{example}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

